StacMR: Scene-Text Aware Cross-Modal Retrieval

Recent models for cross-modal retrieval have benefited from an increasingly rich understanding of visual scenes, afforded by scene graphs and object interactions to mention a few. This has resulted in an improved matching between the visual representation of an image and the textual representation of its caption. Yet, current visual representations overlook a key aspect: the text appearing in images, which may contain crucial information for retrieval. In this paper, we first propose a new dataset that allows exploration of cross-modal retrieval where images contain scene-text instances. Then, armed with this dataset, we describe several approaches which leverage scene text, including a better scene-text aware cross-modal retrieval method which uses specialized representations for text from the captions and text from the visual scene, and reconcile them in a common embedding space. Extensive experiments confirm that cross-modal retrieval approaches benefit from scene text and highlight interesting research questions worth exploring further. Dataset and code are available at http://europe.naverlabs.com/stacmr

==> qualitative_text2image.tex <==
\setlength\tabcolsep{1.2pt}
\begin{figure*}[!t]
% \centering
\begin{center}
\resizebox{\textwidth}{!}
{
\begin{tabular}{c|cccccccccc}
\includegraphics[width=1cm, height=1.35cm, cfbox=blue 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q0.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q1.jpg} & 
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q2.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q3.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q4.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q5.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q6.jpg} & 
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q7.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q8.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n02776631_2689.jpg_q9.jpg} \\

\includegraphics[width=1cm, height=1.35cm, cfbox=blue 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q0.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q1.jpg} & 
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q2.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q3.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q4.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q5.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q6.jpg} & 
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q7.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q8.jpg} &
\includegraphics[width=1cm, height=1.35cm, cfbox=green 1.3pt 0pt]{images/retrieval/context/original/n03039827_2221.jpg_q9.jpg} \\


\end{tabular}
}
\end{center}
\caption{\small Qualitative results in Con-Text Dataset. The first image corresponds to the queried image class. The images are ranked from left to right. Red border represents a mistaken retrieved image that do not correspond to the queried class. (Best viewed in color).}
\label{fig:qualitative_text2image}
\end{figure*}

==> textonly_table.tex <==
\begin{table}[!h]
\begin{center}
\tiny
\setlength\tabcolsep{2pt}
\begin{tabular}{l|rrrrrr|rrrrrr}
\hline
    \multirow{3}{*}{ \textbf{Scene-text Model} }   & \multicolumn{6}{c}{ \textbf{CTC 1k} }                                            & \multicolumn{6}{c}{ \textbf{CTC 5k} }                                           \\
                         
                         & \multicolumn{3}{c}{\textbf{Image to Text}} & \multicolumn{3}{c}{\textbf{Text to Image}} & \multicolumn{3}{c}{\textbf{Image to Text}} & \multicolumn{3}{c}{\textbf{Text to Image}} \\
                         
    & R@1       & R@5       & R@10      & R@1       & R@5       & R@10      & R@1       & R@5       & R@10      & R@1       & R@5       & R@10      \\
\hline
VSE++ GRU                & 17.4      & 29.9      & 37.1      & 8.3       & 17.5      & 23.2      & 2.4       & 4.8       & 5.8       & 1.3       & 3.0       & 4.2       \\
VSRN GRU                 & 7.7       & 18.8      & 26.0      & 5.2       & 12.7      & 18.8      & 1.1       & 2.4       & 3.3       & 0.9       & 2.2       & 3.3       \\
VSE++* GRU               & \textbf{26.3}      & \textbf{40.4}      & \textbf{47.3}      & \textbf{10.0}      & \textbf{20.3}      & \textbf{25.6}      & \textbf{4.4}       & \textbf{7.1}       & \textbf{8.2}       & \textbf{1.6}       & \textbf{3.5}       & \textbf{4.7}       \\
VSRN* GRU                & 12.3      & 25.1      & 30.1      & 6.8       & 15.3      & 20.0      & 1.9       & 4.0       & 5.2       & 1.1       & 2.8       & 3.8       \\
GRU trained on text only & 16.0      & 29.9      & 35.1      & 8.7       & 17.7      & 22.4      & 1.4       & 2.5       & 3.5       & 0.8       & 2.0       & 2.9       \\
fasttext+FV uncleaned    & 19.5      & 35.8      & 43.1      & 0.5       & 1.4       & 2.1       & 3.1       & 5.4       & 7.1       & 0.1       & 0.3       & 0.4       \\
fasttext+FV              & 21.7      & 36.5      & 44.3      & 3.2       & 6.6       & 9.0       & 3.5       & 5.9       & 7.5       & 0.6       & 1.3       & 1.7      
\end{tabular}
\caption{Results on CTC-1k and CTC-5k for several scene-text-only baselines.}
\label{textonly_table}
\end{center}
\end{table}
